SMD-Nets: Stereo Mixture Density Networks

Despite stereo matching accuracy has greatly improved by deep learning in the last few years, recovering sharp boundaries and high-resolution outputs efficiently remains challenging. In this paper, we propose Stereo Mixture Density Networks (SMD-Nets), a simple yet effective learning framework compatible with a wide class of 2D and 3D architectures which ameliorates both issues. Specifically, we exploit bimodal mixture densities as output representation and show that this allows for sharp and precise disparity estimates near discontinuities while explicitly modeling the aleatoric uncertainty inherent in the observations. Moreover, we formulate disparity estimation as a continuous problem in the image domain, allowing our model to query disparities at arbitrary spatial precision. We carry out comprehensive experiments on a new high-resolution and highly realistic synthetic stereo dataset, consisting of stereo pairs at 8Mpx resolution, as well as on real-world stereo datasets. Our experiments demonstrate increased depth accuracy near object boundaries and prediction of ultra high-resolution disparity maps on standard GPUs. We demonstrate the flexibility of our technique by improving the performance of a variety of stereo backbones.

==> tables/HR_ablation.tex <==
\begin{table}[tbp]
\centering
\scalebox{0.68}{
\begin{tabular}{l|c|cc|cc|cc}
\hline
Network  & Input Res. &\multicolumn{3}{c|}{$\SEEk{3}$} & \multicolumn{3}{c|}{$\SEEk{5}$} & \multicolumn{2}{|c}{\EPE} \\
\hline
& & Avg & $\sigma(3)$ & Avg & $\sigma(3)$ & Avg & $\sigma(3)$\\
\hline
HSM \cite{yang2019hierarchical} & $540 \times 960$ & 1.93 & 15.73 & 1.82 & 14.89 & 0.95 & 4.88 \\
HSM* \cite{yang2019hierarchical} + Ours & $540 \times 960$ & \textbf{1.14} & \textbf{5.94} & \textbf{1.03} & \textbf{5.20} & \textbf{0.93} & \textbf{3.84}\\
\hline
HSM \cite{yang2019hierarchical} & $1080 \times 1920$ & 3.30 & 21.96 & 3.03 & 20.44 & \textbf{1.67} & 6.93\\
HSM \cite{yang2019hierarchical}  + SM \cite{chen2019over} & $1080 \times 1920$ & 2.84 & 18.65 & 2.55 & 17.05 & 1.68 & 6.80 \\
HSM* \cite{yang2019hierarchical}  + Ours & $1080 \times 1920$ & \textbf{2.34} & \textbf{12.05} & \textbf{2.09} & \textbf{10.66} & 2.17 & \textbf{6.72}\\
\hline
\end{tabular}
}
\smallskip
\caption{\textbf{Comparison on UnrealStereo4K HR}. We evaluate all methods on ground truth disparity maps of resolution $2160 \times 3840$ \wrt different input resolutions.}
\label{table:hr_ablation}
\end{table}


==> tables/active_data.tex <==
\begin{table}[tp]
\centering
\scalebox{0.70}{
\begin{tabular}{lc|ccc|cc}
\hline
Backbone & Loss  & \multicolumn{3}{|c|}{$SEE_5$} & \multicolumn{2}{|c}{EPE} \\
\hline
& &  & $\sigma(1)$ & $\sigma(3)$ & Avg & $\sigma(3)$\\
\hline
HSM\_single & L1 & 3.40 & \textbf{12.62} & \textbf{6.15} & \textbf{1.58} & \\
HSM\_single & Unimodal \cite{kendall2017uncertainties} & 5.96 & 55.21 & 25.75 & 6.96 & \\
HSM\_single & Bimodal & 4.32 & 27.05 & 13.04 & 4.35 & \\
HSM\_single & Bimodal + DDA & \textbf{3.38} & 19.07 & 8.84 & 2.28 & \\
\hline
HSM\_ext & L1 & 3.40 & \textbf{16.18} & \textbf{6.57} & \textbf{1.60} & \\
HSM\_ext & Unimodal \cite{kendall2017uncertainties} & 5.65 & 50.21 & 21.51 & 6.39 & \\
HSM\_ext & Bimodal & \textbf{3.10} & 30.72 & 8.13 & 2.08 & \\
HSM\_ext & Bimodal + DDA & 3.15 & 16.27 & 7.66 & 2.01 & \\
\hline
\end{tabular}
}
\smallskip
\caption{\textbf{Active data} analysis on the UnrealStereo4K active test set. \cs{consistent network names} \cs{Preliminary numbers, now 20k iterations later, bimodal mostly overtook L1.}}
\label{table:active_ablation}
\end{table}




==> tables/unreal_ablation.tex <==
\begin{table*}[!htbp]
\centering
\scalebox{0.68}{
\begin{tabular}{l|ccc|ccc|ccc|cccccc}
\hline
Network & GT resolution & Sampling & Loss  & \multicolumn{3}{c|}{$SEE_3$} & \multicolumn{3}{c|}{$SEE_5$} & \multicolumn{6}{c}{EPE} \\
\hline
 & & & & Avg & 1px & 3px & Avg & 1px & 3px & Avg & 1px & 2px & 3px & 4px & 5px\\
\hline
PSM \cite{chang2018pyramid} (basic) & $2160 \times 3840$ & - & SmoothL1 & 1.83 & 33.04 & 11.32 & 1.70 & 31.13 & 10.52 & 1.25 & 12.37 & 7.64 & 5.89 & 4.87 & 4.19\\
PSM \cite{chang2018pyramid} (stack-hourglass) & $2160 \times 3840$ & - & SmoothL1 & - & - & - & - & - & - & - & - & - & - & - & -\\
PSM \cite{chang2018pyramid} (stack-hourglass) + \cite{chen2019over} & $2160 \times 3840$ & - & SmoothL1 & - & - & - & - & - & - & - & - & - & - & - & -\\
PSM \cite{chang2018pyramid} (stack-hourglass) + Median Filter & $2160 \times 3840$ & - & SmoothL1 & - & - & - & - & - & - & - & - & - & - & - & -\\
HSM \cite{yang2019hierarchical} & $2160 \times 3840$ & - & SmoothL1 & 1.93 & 41.38 & 15.73 & 1.82 & 39.47 & 14.89 & 0.95 & 12.80 & 7.00 & 4.88 & 3.70 & 2.97\\
HSM \cite{yang2019hierarchical}  + Single-Modal \cite{chen2019over} & $2160 \times 3840$ & - & SmoothL1 & 1.72 & 40.13 & 13.92 & 1.60 & 38.16 & 13.04 & 0.95 & 12.75 & 6.93 & 4.80 & 3.62 & 2.90\\
HSM \cite{yang2019hierarchical} + Median Filter & $2160 \times 3840$ & - & SmoothL1 & 1.94 & 41.45 & 15.80 & 1.83 & 39.55 & 14.95 & 0.95 & 12.78 & 6.99 & 4.87 & 3.69 & 2.97\\
Ours & $2160 \times 3840$ & Random & L1 & 1.71 & 35.46 & 12.37 & 1.60 & 33.48 & 11.53 & 1.04 & 13.62 & 7.21 & 5.06 & 3.91 & 3.20\\
Ours & $2160 \times 3840$ & Random & Unimodal \cite{kendall2017uncertainties} & 2.37 & 41.76 & 18.17 & 2.25 & 39.96 & 17.33 & 1.64 & 16.01 & 10.08 & 7.73 & 6.38 & 5.48\\
Ours & $2160 \times 3840$ & Random & Bimodal & 1.32 & 25.93 & 7.27 & 1.19 & 23.87 & 6.41  & 0.99 & 10.58 & 5.81 & 4.18 & 3.29 & 2.76\\
Ours & $2160 \times 3840$ & DDA & Bimodal & \textbf{1.14} & \textbf{22.46} & \textbf{5.94} & \textbf{1.03} & \textbf{20.54} & \textbf{5.20} & \textbf{0.93} & \textbf{10.27} & \textbf{5.44} & \textbf{3.84} & \textbf{3.02} & \textbf{2.53}\\
Ours (2D backbone) & $2160 \times 3840$ & DDA & Bimodal & 1.42 & 27.60 & 8.34 & 1.30 & 25.70 & 7.56 & 1.28 & 17.08 & 8.69 & 5.97 & 4.58 & 3.76\\
\hline
PSM \cite{chang2018pyramid} (basic)  & $540 \times 960$ & - & SmoothL1 & 1.72 & 30.47 & 10.48 & 1.47 & 26.70 & 9.01 & 1.24 & 12.25 & 7.59 & 5.85 & 4.84 & 4.17\\
PSM \cite{chang2018pyramid} (stack-hourglass) & $540 \times 960$ & - & SmoothL1 & - & - & - & - & - & - & - & - & - & - & - & -\\
HSM \cite{yang2019hierarchical} & $540 \times 960$ & - & SmoothL1 & 1.79 & 38.66 & 14.37 & 1.57 & 34.87 & 12.84 & 0.94 & 12.70 & 6.96 & 4.85 & 3.68 & 2.96\\
Ours & $540 \times 960$ & Random & Bimodal & 1.20 & 22.90 & 6.32 & 0.97 & 18.80 & 4.83 & 0.97  & 10.68 & 5.89 & 4.26 & 3.36 & 2.82\\
Ours & $540 \times 960$ & DDA & Bimodal & 1.09 & 19.67 & 5.49 & 0.88 & 16.01 & 4.30 & 0.95  & 10.54 & 5.62 & 3.99 & 3.15 & 2.65\\
\hline
\end{tabular}
}
\smallskip
\caption{\textbf{Ablation study} of our Mixture Density Stereo Network (MDS-Net) on the UnrealStereo4K test set. (In-Domain)}
\label{table:ablation}
\end{table*}



\begin{table*}[!htbp]
\centering
\scalebox{0.68}{
\begin{tabular}{l|ccc|ccc|ccc|cccccc}
\hline
Network & GT resolution & Sampling & Loss  & \multicolumn{3}{|c|}{$SEE_3$} & \multicolumn{3}{|c|}{$SEE_5$} & \multicolumn{6}{|c}{EPE} \\
\hline
 & & & & Avg & 1px & 3px & Avg & 1px & 3px & Avg & 1px & 2px & 3px & 4px & 5px\\
\hline
PSM \cite{chang2018pyramid} (basic)  & $2160 \times 3840$ & - & SmoothL1 & 2.34 & 36.49 & 14.24 & 2.13 & 33.38 & 12.89 & 1.71 & \textbf{16.96} & 10.63 & 8.29 & 6.97 & 6.08\\
PSM \cite{chang2018pyramid} (stack-hourglass) & $2160 \times 3840$ & - & SmoothL1 & - & - & - & - & - & - & - & - & - & - & - & -\\
HSM \cite{yang2019hierarchical} & $2160 \times 3840$ & - & SmoothL1 & 2.29 & 43.92 & 17.37 & 2.11 & 41.19 & 16.04 & \textbf{1.45} & 19.85 & 11.43 & 8.27 & 6.56 & 5.45\\
HSM \cite{yang2019hierarchical}  + Single-Modal \cite{chen2019over} & $2160 \times 3840$ & - & SmoothL1 & 2.15 & 43.11 & 16.19 & 1.95 & 40.33 & 14.83 & 1.45 & 19.74 & 11.29 & 8.12 & 6.40 & 5.59\\
Ours & $2160 \times 3840$ & Random & L1 & 2.38 & 42.68 & 16.65 & 2.20 & 39.94 & 15.32 & 1.61 & 21.38 & 12.21 & 8.83 & 7.05 & 5.91\\
Ours & $2160 \times 3840$ & Random & Unimodal \cite{kendall2017uncertainties} & 2.94 & 46.05 & 20.85 & 2.74 & 43.45 & 19.50 & 2.05 & 36.27 & 23.16 & 23.16 & 14.57 & 11.10\\
Ours & $2160 \times 3840$ & Random & Bimodal & 2.10 & 35.00 & 11.92 & 1.89 & 32.06 & 10.5 & 1.61 & 17.78 & 10.21 & 7.54 & 6.19 & 5.35\\
Ours & $2160 \times 3840$ & DDA & Bimodal & \textbf{1.86} & \textbf{33.43} & \textbf{10.73} & \textbf{1.67} & \textbf{30.54} & \textbf{9.41} & 1.49 & 17.75 & \textbf{9.92} & \textbf{7.20} & \textbf{5.82} & \textbf{4.94}\\
\hline
\end{tabular}
}
\smallskip
\caption{\textbf{Ablation study} of our Mixture Density Stereo Network (MDS-Net) on the UnrealStereo4K test set. (Out-domain) TEMPORARY TABLE.}
\label{table:ablation}
\end{table*}

